Accelerating JavaScript Static Analysis via Dynamic Shortcuts (Extended Version)

JavaScript has become one of the most widely used programming languages for web development, server-side programming, and even micro-controllers for IoT. However, its extremely functional and dynamic features degrade the performance and precision of static analysis. Moreover, the variety of built-in functions and host environments requires excessive manual modeling of their behaviors. To alleviate these problems, researchers have proposed various ways to leverage dynamic analysis during JavaScript static analysis. However, they do not fully utilize the high performance of dynamic analysis and often sacrifice the soundness of static analysis. In this paper, we present dynamic shortcuts, a new technique to flexibly switch between abstract and concrete execution during JavaScript static analysis in a sound way. It can significantly improve the analysis performance and precision by using highly-optimized commercial JavaScript engines and lessen the modeling efforts for opaque code. We actualize the technique via $\text{SAFE}_\textsf{DS}$, an extended combination of $\text{SAFE}$ and Jalangi, a static analyzer and a dynamic analyzer, respectively. We evaluated $\text{SAFE}_\textsf{DS}$ using 269 official tests of Lodash 4 library. Our experiment shows that $\text{SAFE}_\textsf{DS}$ is 7.81x faster than the baseline static analyzer, and it improves the precision to reduce failed assertions by 12.31% on average for 22 opaque functions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=main


PDF = $(PACKAGE).pdf

all: pdf

pdf:
	pdflatex $(PACKAGE)
	- bibtex $(PACKAGE)
	pdflatex $(PACKAGE)
	pdflatex $(PACKAGE)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(PACKAGE).log) \
	do pdflatex $(PACKAGE); done

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

clean: docclean

distclean: clean
	$(RM)  *.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ main.pdf ACM-Reference-Format.*

.PHONY: all docclean clean distclean archive zip
.SILENT: pdf


==> def.tex <==
\section{Definition of Dynamic Shortcut}\label{sec:def}

In this section, we introduce the formal definition of dynamic shortcut based on
sealed symbolic execution in abstract interpretation.



\subsection{Abstract Interpretation}

We first define the traditional abstract interpretation.


\subsubsection{Concrete Semantics}

We define a program $\prog$ as a state transition system $(\stset, \trans,
\istset)$.  A program starts with an initial state in $\istset$ and the
transition relation $\trans \subseteq \stset \times \stset$ describes how states
are transformed to other states.  A \textit{collecting semantics} $\sem{\prog} =
\{ \st \in \stset \mid \ist \in \istset \wedge \ist \trans^* \st \}$ consists of
reachable states from initial states of the program $\prog$.  We could calculate
it using the \textit{transfer function} $\transfer: \dom \rightarrow \dom$ as
follows:
\[
  \sem{\prog} = \underset{n \rightarrow \infty}{\lim}{\transfer^n(\ielem)}\\
  \qquad
  \transfer(\elem) = \elem \join \step(\elem)\\
\]
The \textit{concrete domain} $\dom = \powerset{\stset}$ is a complete lattice
with $\cup$, $\cap$, and $\subseteq$ as its join($\join$), meet($\meet$), and
partial order($\order$) operators.  The set of states $\ielem$ denotes the
initial states $\istset$.  The \textit{one-step execution} $\step: \dom
\rightarrow \dom$ transforms states using the transition relation $\trans$:
$\step(\elem) = \{ \st' \mid \st \in \elem \wedge \st \trans \st' \}$.


\subsubsection{Abstract Interpretation}

The abstract interpretation over-approximates the transfer $\transfer$ to the
\textit{abstract transfer function} $\abstransfer: \absdom \rightarrow \absdom$
to get the \textit{abstract semantics} $\abssem{\prog}$ in finite iterations as
follows:
\[
    \abssem{\prog} = \underset{n \rightarrow
    \infty}{\lim}{(\abstransfer)^n(\iabselem)}\\
\]
We define a \textit{state abstraction} $\dom \galois{\alpha}{\gamma} \absdom$ as
a Galois connection between the concrete domain $\dom$ and an abstract domain
$\absdom$ with a \textit{concretization function} $\gamma$ and an
\textit{abstraction function} $\alpha$.  The initial abstract state $\iabselem
\in \absdom$ represents an abstraction of the initial state set; $\ielem
\subseteq \gamma(\iabselem)$.  The abstract transfer function $\abstransfer:
\absdom \rightarrow \absdom$ is defined as $\abstransfer(\abselem) = \abselem
\join \absstep(\abselem)$ with an \textit{abstract one-step execution}
$\absstep: \absdom \rightarrow \absdom$.  For the sound state abstraction, the
join operator and the abstract one-step execution should satisfy the following
conditions:
\begin{equation}\label{equ:sound}
  \begin{array}{l}
  - \; \forall \abselem_0, \abselem_1 \in \absdom. \; \gamma(\abselem_0) \cup
    \gamma(\abselem_1) \subseteq \gamma(\abselem_0 \join \abselem_1)\\
  - \; \forall \abselem \in \absdom. \; \step \circ \gamma(\abselem) \subseteq
    \gamma \circ \absstep(\abselem)\\
  \end{array}
\end{equation}


\subsubsection{Analysis Sensitivity}

Abstract interpretation is often defined with \textit{analysis sensitivity} to
increase the precision of static analysis.  A sensitive abstract domain
$\sabsdom: \viewset \rightarrow \absdom$ is defined with a \textit{view
abstraction} $\viewmap: \viewset \rightarrow \dom$ that provides multiple points
of views for reachable states during static analysis.  It maps a finite number
of views $\viewset$ to sets of states $\dom$. Each view $\view \in \viewset$
represents a set of states $\viewmap(\view)$ and also a state is always
included in a unique view: $\forall \st \in \stset. \; \exists! \view \in
\viewset.$ s.t. $\st \in \viewmap(\view)$.  A \textit{sensitive state
abstraction} $\dom \galois{\alpha_\viewmap}{\sgamma} \sabsdom$ is a Galois
connection between the concrete domain $\dom$ and the sensitive abstract domain
$\sabsdom$ with the following concretization function:
\[
  \sgamma(\sabselem) = \underset{\view \in \viewset}{\bigcup}
  {\viewmap(\view) \cap \gamma \circ \sabselem(\view)}
\]

With analysis sensitivities, the abstract one-step execution $\sabsstep:
\sabsdom \rightarrow \sabsdom$ is defined as follows:
\[
  \sabsstep(\sabselem) = \lambda \view \in \viewset. \; \underset{\view' \in
  \viewset}{\bigjoin}{\viewtrans{\view'}{\view} \circ \sabselem(\view')}
\]
where $\viewtrans{\view'}{\view}: \absdom \rightarrow \absdom$ is the abstract
semantics of a \textit{view transition} from a view $\view'$ to another view
$\view$.  It should satisfy the following condition for the soundness of the
analysis:
\[
  \forall \abselem \in \absdom. \; \step(\gamma(\abselem) \cap \viewmap(\view'))
  \cap \viewmap(\view) \subseteq \gamma \circ
  \viewtrans{\view'}{\view}(\abselem)
\]



\subsection{Dynamic Shortcut}

We define dynamic shortcut by combining the sensitive abstract interpretation
with sealed symbolic execution.


\subsubsection{Sealed Symbolic Execution}

We define \textit{sealed symbolic execution} by extending the transition
relation $\trans$ as a symbolic transition relation $\symbtrans$ on symbolic
states.  First, we augment concrete states $\stset$ to symbolic states
$\symbstset$ by extending values $\valset$ with \textit{sealed symbolic values}
$\symbset$.  We also define the symbolic transition relation $\symbtrans
\subseteq \symbstset \times \symbstset$. We use the notation $\symbtrans^k$
for $k$ repetition of $\symbtrans$, and  $\symbst \symbtrans \excst$ when
$\symbst$ does not have symbolic transitions with any other symbolic states.  We
also define the soundness of sealed symbolic execution as follows:
\begin{definition}{(Validity)}
  The symbolic transition relation is \textit{valid} when the following
  condition is satisfied:
  \[
      \forall \symbst, \symbst' \in \symbstset.\\
  \]
  \[
    \symbst \symbtrans \symbst' \Leftrightarrow
    \forall \imap \in \imapset. \;
    \{ \st' \mid \instant{\symbst}{\imap} \trans \st' \}
    = \{ \instant{\symbst'}{\imap} \}
  \]
  where $\imapset: \symbset \rightarrow \valset$ is instantiation maps from
  symblic values to real values, and $\instant{\symbst}{\imap}$ denotes a state
  produced by replacing each symbolic value $\symb$ to the corresponding value
  $\imap(\symb)$ using the instantiation map $\imap \in \imapset$.
\end{definition}

Note that the main difference of sealed symbolic execution with the traditional
symbolic execution is that it only supports sealed symbolic values instead of
symbolic expressions and path constraints.

We also define an \textit{abstract instantiation map} $\absimap \in \absimapset:
\symbset \rightarrow \absvalset$ with abstract values $\absvalset$.  Its
concretization function $\imapgamma: \absimapset \rightarrow
\powerset{\imapset}$ is defined with the concretization function $\valgamma:
\absvalset \rightarrow \powerset{\valset}$ for values as follows:
\[
  \imapgamma(\absimap) = \{
    \imap \mid \forall \symb \in \symbset. \;
    \imap(\symb) \in \gamma \circ \absimap(\symb)
  \}
\]
We define the instantiation of a given sealed symbolic state $\symbst \in
\symbstset$ with an abstract instantiation map $\absimap \in \absimapset$ as
follows:
\[
  \instant{\symbst}{\absimap} = \{ \instant{\symbst}{\imap} \mid \imap \in
  \imapgamma(\absimap) \}
\]

\begin{definition}[Sealed Symbolic Domain]
  We define \textit{sealed symbolic domain} $\symbdom: \powerset{\absimapset
  \times \symbstset}$ with the following concretization function $\symbgamma:
  \symbdom \rightarrow \dom$ and sealed symbolic one-step execution $\symbstep:
  \symbdom \rightarrow \symbdom$ as follows:
  \begin{itemize}
    \item \(
      \symbgamma(\symbelem) = 
      \bigcup \{ \instant{\symbst}{\absimap} \mid (\absimap, \symbst) \in
      \symbelem\}
    \)
    \item \(
      \symbstep(\symbelem) = \{ (\absimap, \symbst') \mid (\absimap, \symbst)
      \in \symbelem \wedge \symbst \symbtrans \symbst' \}
    \)
  \end{itemize}
\end{definition}


\subsubsection{Combined Domain}

\begin{definition}[Combined Domain]
  We define a \textit{combined domain} as $\combdom = \sabsdom \times \symbdom$
  with the following concretization function and join operator:
  \begin{itemize}
    \item \(
      \combgamma((\sabselem, \symbelem)) = \sgamma(\sabselem) \cup
      \symbgamma(\symbelem)
    \)
    \item \(
      (\sabselem, \symbelem) \join ({\sabselem}', \symbelem') = (\sabselem \join
      {\sabselem}', \symbelem \cup \symbelem')
    \)
  \end{itemize}
\end{definition}

An analysis element $\aelem \in \aelemset = (\viewset \times \absdom) \uplus
(\absimapset \times \symbstset)$ is either a pair of a view and an abstract
state or a sealed symbolic state.  To freely convert a pair of a view and an
abstract state to its corresponding pair of an abstract instantiation map and a
sealed symbolic state, we define two domain converters: \begin{itemize} \item
$\asconverter: (\viewset \times \absdom) \hookrightarrow (\absimapset \times
\symbstset)$ \item $\saconverter: (\viewset \times \absdom) \leftarrow
(\absimapset \times \symbstset)$ \end{itemize} The converter $\asconverter$ is a
\textit{partial function} and it is applicable when it is possible to represent
a given abstract state in a specific view as a pair of abstract instantiation
map and a sealed symbolic state.  We define the concretization function
$\aelemgamma: \aelemset \rightarrow \dom$ for analysis elements as follows:
\[
  \aelemgamma(\aelem) = \left\{
    \begin{array}{ll}
      \viewmap(\view) \cap \gamma(\abselem) & \text{if} \; (\view, \abselem) = \aelem\\
      \instant{\symbst}{\absimap} & \text{if} \; (\absimap, \symbst) = \aelem\\
    \end{array}
  \right.
\]
Moreover, two converters should convert given elements without loss of
information:
\[
  \forall \view \in \viewset, \abselem \in \absdom.
\]
\[
  \asconverter(\aelem) = \aelem' \Rightarrow \left\{
  \begin{array}{l}
    \aelem = \saconverter(\aelem')\\
    \aelemgamma(\aelem) = \aelemgamma(\aelem')\\
  \end{array}
  \right.
\]

We define a $\areform$ function using two converters between analysis elements
as follows:
\begin{definition}[$\areform$]\label{def:areform}
  The reform function $\areform: \aelemset \rightarrow \aelemset$ for analysis
  elements is defined as
  \[
    \areform(\aelem) = \left\{
      \begin{array}{ll}
        \asconverter(\aelem)
        & \text{if} \; \aelem = (\view, \abselem) \wedge \aelem \in
        \Dom(\asconverter)\\
        \saconverter(\aelem)
        & \text{if} \; \aelem = (\absimap, \symbst) \wedge \symbst \symbtrans
        \bot\\
        \aelem
        & \text{Otherwise}
      \end{array}
    \right.
  \]
\end{definition}
Using the $\areform$ function for analysis elements, we defined the $\reform$
function for combined states:
\begin{definition}[$\reform$]\label{def:reform}
  The reform function $\reform: \combdom \rightarrow \combdom$ for combined
  states is defined as
  \[
    \reform((\sabselem, \symbelem)) = \left(
      \lambda \view. \bigjoin \{ \abselem \!\mid\! (\view, \abselem) \in E \},
      E \cap (\absimapset \times \symbstset)
    \right)
  \]
  where
  \[
    E = \dot{\areform}(\{ (\view, \sabselem(\view)) \mid \view \in \viewset \} \cup \symbelem)
  \]
\end{definition}
The dot notation $\dot{f}$ denotes the element-wise extended function of a
function $f$.

\begin{definition}[Combined One-Step Execution]
  We define the combined one-step execution $\combstep: \combdom \rightarrow
  \combdom$ is define as follows:
  \[
    \combstep(\combelem) = (
      \sabsstep(\sabselem),
      \symbstep(\symbelem)
    )
  \]
  where $(\sabselem, \symbelem) = \reform(\combelem)$.
\end{definition}

We could configure when the sealed symbolic execution or the abstract
interpretation is performed based on the definition of the converter
$\asconverter$.  For example, we could define the $\asconverter$ for analysis
elements related to only function entry, call, and exit points to perform
conversions in a function level.  For the soundness and the termination of the
the abstract interpretation with dynamic shortcuts, it should satisfy the
following condition:
\begin{theorem}[Soundness and Termination]\label{theorem:shortcut}
  The abstract interpretation with dynamic shortcut is sound and terminates in a
  finite time if its abstract semantics is sound and $\saconverter$ satisfies the
  following condition:
  \begin{equation}\label{equ:asc-cond}
    \asconverter((\view, \abselem)) = (\absimap, \symbst) \Rightarrow
    \symbst \symbtrans^k \excst \wedge 1 < k \leq N
  \end{equation}
  where $N$ is a pre-defined maximum length of the sealed symbolic execution.
\end{theorem}

In the remaining section, we will prove this theorem using the Kleene's
fixed-point theorem with the finite height of abstract domains.


==> macros.tex <==
% latexdiff
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}} %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

% thicker vertical line
\newcolumntype{?}{!{\vrule width 1pt}}

% Styles
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\lstdefinelanguage{JavaScript}{
  keywords={async, await, break, case, catch, class, const, continue, debugger,
    default, delete, do, else, enum, export, extends, false, finally, for,
    function, if, import, in, instanceof, new, null, return, super, switch, this,
    throw, true, try, typeof, var, void, while, with, yield},
  keywordstyle=\color{blue}\bfseries,
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{dkgreen}\ttfamily,
  stringstyle=\color{purple}\ttfamily,
  morestring=[b]',
  morestring=[b]"
}
\lstdefinestyle{myJSstyle}{
  language=JavaScript,
  numbers=left,
  stepnumber=1,
  extendedchars=true,
  basicstyle=\footnotesize\ttfamily,
  showstringspaces=false,
  showspaces=false,
  xleftmargin=\parindent,
  tabsize=2,
  breaklines=true,
  showtabs=false,
  captionpos=b
}
\lstdefinelanguage{nJavaScript}{
  keywordstyle=\color{blue}\bfseries,
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{dkgreen}\ttfamily,
  stringstyle=\color{purple}\ttfamily,
  morestring=[b]',
  morestring=[b]"
}
\lstdefinestyle{nmyJSstyle}{
  language=nJavaScript,
  numbers=left,
  stepnumber=1,
  extendedchars=true,
  basicstyle=\footnotesize\ttfamily,
  showstringspaces=false,
  showspaces=false,
  xleftmargin=\parindent,
  tabsize=2,
  breaklines=true,
  showtabs=false,
  captionpos=b
}

% Basic
\DeclareMathAlphabet{\mathpzc}{T1}{pzc}{m}{it}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}
\newcommand{\imbox}[1]{\mbox{\small \textit{#1}}}
\newcommand{\name}[1]{\textsf{#1}}
\newcommand{\inred}[1]{{\color{red}{#1}}}
\newcommand{\todo}{\inred{TODO}}
\newcommand{\abs}[1]{{#1}^{\#}}
\newcommand{\finmap}{{\xrightarrow[]{\text{fin}}}}
\newcommand{\mapstos}{\;\dot{\mapsto}\;}
\newcommand{\Dom}{\name{Dom}}

% Tool
\newcommand{\tool}{\text{SAFE}_\name{DS}}

% Keywords
\newcommand{\jscode}[1]{\text{\lstinline[style=myJSstyle,numbers=none]!#1!}}
\newcommand{\njscode}[1]{\text{\lstinline[style=nmyJSstyle,numbers=none]!#1!}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\kwif}{\code{if}}
\newcommand{\kwelse}{\code{else}}
\newcommand{\kwret}{\code{ret}}
\newcommand{\kwobj}{\code{\{\}}}
\newcommand{\kwtrue}{\code{true}}
\newcommand{\kwfalse}{\code{false}}

% Notations
\newcommand{\prog}{P}
\newcommand{\labset}{\mathcal{L}}
\newcommand{\lab}{\mathpzc{l}}
\newcommand{\labdot}[1]{{{\bullet_{\lab_{#1}}}}}
\newcommand{\ilab}{\lab_\iota}
\newcommand{\labnext}{\name{next}}
\newcommand{\op}{\name{op}}
\newcommand{\ops}{\dot{\name{op}}}
\newcommand{\inst}{i}
\newcommand{\expr}{e}
\newcommand{\refer}{r}

% Numbers
\newcommand{\numset}{\mathbb{N}}

% States
\newcommand{\stset}{\mathbb{S}}
\newcommand{\st}{\sigma}
\newcommand{\istset}{\stset_\iota}
\newcommand{\ist}{\st_\iota}

% Memories
\newcommand{\memset}{\mathcal{M}}
\newcommand{\absmemset}{\abs{\memset}}
\newcommand{\mem}{M}
\newcommand{\absmem}{\abs{\mem}}

% Contexts
\newcommand{\ctxtset}{\mathbb{C}}
\newcommand{\absctxtset}{\abs{\ctxtset}}
\newcommand{\ctxt}{c}
\newcommand{\absctxt}{\abs{\ctxt}}
\newcommand{\eabsctxt}{\absctxt_\name{env}}

% Transition Relations
\newcommand{\trans}{\leadsto}
\newcommand{\rutrans}{%
            \mathrel{\raisebox{.1em}{%
            \rotatebox[origin=c]{30}{$\trans$}}}}
\newcommand{\rdtrans}{%
            \mathrel{\raisebox{.1em}{%
            \rotatebox[origin=c]{-30}{$\trans$}}}}


% Complete Lattice
\newcommand{\join}{\sqcup}
\newcommand{\meet}{\sqcap}
\newcommand{\bigjoin}{\bigsqcup}
\newcommand{\bigmeet}{\bigsqcap}
\newcommand{\order}{\sqsubseteq}

% Concrete Domains
\newcommand{\dom}{\mathbb{D}}
\newcommand{\elem}{d}
\newcommand{\ielem}{\elem_\iota}

% Abstract Domains
\newcommand{\absdom}{\abs{\dom}}
\newcommand{\abselem}{\abs{\elem}}
\newcommand{\iabselem}{\abs{\elem}_\iota}

% Concrete Semantics
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\transfer}{F}
\newcommand{\step}{\name{step}}

% Abstract Semantics
\newcommand{\abssem}[1]{\abs{\sem{#1}}}
\newcommand{\abstransfer}{\abs{\transfer}}
\newcommand{\absstep}{\abs{\step}}

% Abstract Sensitivity
\newcommand{\viewmap}{\delta}
\newcommand{\sabsdom}{\absdom_\viewmap}
\newcommand{\sabselem}{{\abselem_\viewmap}}
\newcommand{\isabselem}{{\abs{\elem}_\viewmap}_\iota}
\newcommand{\viewset}{\Pi}
\newcommand{\view}{\pi}
\newcommand{\sabsstep}{\absstep_\viewmap}
\newcommand{\viewtrans}[2]{\abssem{#1 \rightarrow #2}}

% Flow Sensitivity
\newcommand{\fs}{\name{FS}}
\newcommand{\fsviewmap}{\viewmap^\fs}

% Locations
\newcommand{\locset}{\mathbb{L}}
\newcommand{\loc}{l}
\newcommand{\abslocset}{\abs\locset}
\newcommand{\absloc}{\abs\loc}

% Variables
\newcommand{\varset}{\mathbb{X}}
\newcommand{\varx}{\code{x}}

% Values
\newcommand{\valset}{\mathbb{V}}
\newcommand{\val}{v}
\newcommand{\pvalset}{\valset_\name{p}}
\newcommand{\pval}{\val_\name{p}}
\newcommand{\fvalset}{\mathbb{F}}
\newcommand{\fval}[2]{\lambda #1. #2}
\newcommand{\strset}{\valset_\name{str}}
\newcommand{\str}{\val_\name{str}}
\newcommand{\absvalset}{\abs{\valset}}
\newcommand{\absval}{\abs{\val}}

\newcommand{\valgamma}{\gamma_\val}

% Addresses
\newcommand{\addrset}{\mathbb{A}}
\newcommand{\eaddrset}{\addrset_\name{env}}
\newcommand{\oaddrset}{\addrset_\name{obj}}
\newcommand{\addr}{a}
\newcommand{\tladdr}{\addr_{\name{top}}}
\newcommand{\absaddrset}{\abs{\addrset}}
\newcommand{\absaddr}{\abs{\addr}}
\newcommand{\eabsaddr}{\absaddr_\name{env}}
\newcommand{\rabsaddr}{\absaddr_\name{ret}}
\newcommand{\oabsaddr}{\absaddr_\name{obj}}

% Abstract Counting
\newcommand{\abscount}{\abs{n}}
\newcommand{\inc}{\name{inc}}
\newcommand{\abscountset}{\abs{\mathbb{N}}}
\newcommand{\abszero}{\abs{0}}
\newcommand{\absone}{\abs{1}}
\newcommand{\absmany}{\abs{\geq\!\!2}}

% Sealed Symbolic Interpretation
\newcommand{\sealed}{sealed}
\newcommand{\Sealed}{Sealed}
\newcommand{\SealeD}{Sealed}
\newcommand{\symb}{\omega}
\newcommand{\symbset}{\Omega}
\newcommand{\symbolic}[1]{{#1}_\symb}
\newcommand{\symbstset}{\symbolic{\stset}}
\newcommand{\symbst}{\symbolic{\st}}
\newcommand{\nsymbst}[1]{\st_{\symb,#1}}
\newcommand{\symbmemset}{\symbolic{\memset}}
\newcommand{\symbtrans}{\symbolic{\trans}}
\newcommand{\excst}{\bot}
\newcommand{\symbevt}{\symb_\jscode{evt}}
\newcommand{\symbint}{\symb_\jscode{int}}

% Combined Analysis
\newcommand{\comb}[1]{\widetilde{#1}}
\newcommand{\combdom}{\comb{\dom}}
\newcommand{\combelem}{\comb{\elem}}
\newcommand{\icombelem}{\comb{\elem}_\iota}
\newcommand{\combgamma}{\comb{\gamma}}
\newcommand{\combstep}{\comb{\step}}
\newcommand{\combtransfer}{\comb{\transfer}}
\newcommand{\combsem}[1]{\comb{\sem{#1}}}
\newcommand{\sgamma}{\gamma_\viewmap}
\newcommand{\converter}{\tau}
\newcommand{\saconverter}{\abs{\converter}}
\newcommand{\asconverter}{\symbolic{\converter}}
\newcommand{\combviewtrans}[2]{\sem{\comb{#1 \rightarrow #2}}}

\newcommand{\symbdom}{\symbolic{\dom}}
\newcommand{\symbelem}{{\symbolic{\elem}}}
\newcommand{\symbgamma}{\symbolic{\gamma}}
\newcommand{\symbstep}{\symbolic{\step}}

% Reform
\newcommand{\reformname}{reform\xspace}
\newcommand{\reform}{\name{\reformname}}
\newcommand{\areform}{\reform_\aelem}

% Rules
\newcommand{\referrule}[3]{#1 \vdash_\refer #2 \Rightarrow  #3}
\newcommand{\exprrule}[3]{#1 \vdash_\expr #2 \Rightarrow #3}

% Abstract Semantics
\newcommand{\referabssem}[1]{\abssem{#1}_\refer}
\newcommand{\exprabssem}[1]{\abssem{#1}_\expr}

% Identity function
\newcommand{\identity}{\name{id}}

% Checker
\newcommand{\checker}{\name{checker}\xspace}

% Concerto
\newcommand{\concerto}{\textsc{Concerto}\xspace}

% Table 1
\newcommand{\myhead}[3]{
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#1}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#2}}} &
  \multicolumn{2}{c?}{\textbf{#3}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#1}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#2}}} &
  \multicolumn{2}{c?}{\textbf{#3}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#1}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{#2}}} &
  \multicolumn{2}{c}{\textbf{#3}}
  \\\cline{3-4}\cline{7-8}\cline{11-12}

  && \textbf{orig.} & \textbf{abs.} &
  && \textbf{orig.} & \textbf{abs.} &
  && \textbf{orig.} & \textbf{abs.}\\\hline
}
\newcommand{\mysuff}[5]{
  \multirow{#1}{*}{\jscode{#2}} &
  \jscode{#3} &
  \text{#4} &
  \text{#5}
}
\newcommand{\mysucccolor}{yellow}

\newcommand{\mnsutf}[5]{
  \multirow{#1}{*}{\njscode{#2}} &
  {\jscode{#3}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c|}    {\text{#4}} &
  {\text{#5}}
}
\newcommand{\mysutf}[5]{
  \multirow{#1}{*}{\jscode{#2}} &
  {\jscode{#3}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c|}    {\text{#4}} &
  {\text{#5}}
}
\newcommand{\mysuft}[5]{
  \multirow{#1}{*}{\jscode{#2}} &
  {\jscode{#3}} &
  {\text{#4}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c?}    {\text{#5}}
}
\newcommand{\mysutt}[5]{
  \multirow{#1}{*}{\jscode{#2}} &
  {\jscode{#3}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c|}    {\text{#4}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c?}    {\text{#5}}
}
\newcommand{\mysbtt}[5]{
  \multirow{#1}{*}{\jscode{#2}} &
  {\jscode{#3}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c|}    {\text{#4}} &
  \multicolumn{1}{>{\columncolor{\mysucccolor}}c}    {\text{#5}}
}

\newcommand{\mylinef}  {\\\hhline{~|---}}
\newcommand{\mylineff} {\\\hhline{~|---~|---}}
\newcommand{\mylinetf} {\\\hhline{----~|---}}
\newcommand{\mylinefff}{\\\hhline{~|---~|---~|---}}
\newcommand{\mylinefft}{\\\hhline{~|---~|-------}}
\newcommand{\mylineftf}{\\\hhline{~|-------~|---}}
\newcommand{\mylineftt}{\\\hhline{~|-----------}}
\newcommand{\mylinetff}{\\\hhline{----~|---~|---}}
\newcommand{\mylinetft}{\\\hhline{----~|-------}}
\newcommand{\mylinettf}{\\\hhline{--------~|---}}
\newcommand{\mylinettt}{\\\hhline{------------}}

% Instantiation Map
\newcommand{\imap}{m}
\newcommand{\imapset}{\mathbb{M}}
\newcommand{\absimap}{\abs{\imap}}
\newcommand{\absimapset}{\abs{\imapset}}
\newcommand{\instant}[2]{#1\!\!\mid\!\!_{#2}}
\newcommand{\imapgamma}{\gamma_\imap}

% Analysis Element
\newcommand{\aelem}{\epsilon}
\newcommand{\aelemset}{\mathbb{E}}
\newcommand{\aelemgamma}{\gamma_{\aelem}}

% Termination
\newcommand{\symbaelem}{\symbolic{\aelem}}
\newcommand{\liftsymbtrans}{\hat\trans_\symb}
\newcommand{\diffset}{\Delta}
\newcommand{\ttl}{\name{TTL}}

% speed up
\newcommand{\x}{{\textsf{x}}}


==> proof.tex <==
\section{Proof of Theorem 1.4}\label{sec:proof}

We formally rephrase the meaning of Theorem~\ref{theorem:shortcut} in
Theorem~\ref{theorem:soundness} and Theorem~\ref{theorem:termination}.  Now, we
assume that the baseline sensitive abstract domain ensures the soundness and
satisfies ascending chain condition, the sealed symbolic execution is valid,
and the converter $\asconverter: (\viewset \times \absdom) \hookrightarrow
(\absimapset \times \symbstset)$ satisfies the
condition~(\ref{equ:asc-cond}) in the Theorem~\ref{theorem:shortcut}.


\subsection{Soundness}

\begin{theorem}[Soundness]\label{theorem:soundness}
  The abstract interpretation using the combined domain $\combdom$ is
  \textit{sound} if and only if
  \begin{equation}\label{equ:comb-sound1}
    \forall \combelem_0, \combelem_1 \in \combdom. \; \combgamma(\combelem_0) \cup
    \combgamma(\combelem_1) \subseteq \combgamma(\combelem_0 \join \combelem_1)
  \end{equation}
  \begin{equation}\label{equ:comb-sound2}
    \forall \combelem \in \combdom. \; \step \circ \combgamma(\combelem) \subseteq
    \combgamma \circ \combstep(\combelem)\\
  \end{equation}
\end{theorem}
\begin{proof}
  First, we prove that the abstract transfer function $\combtransfer: \combdom
  \rightarrow \combdom$ defined as $\combtransfer(\combelem) = \combelem \join
  \combstep(\combelem)$ is sound
  \[
    \begin{array}{rcll}
      \transfer \circ \combgamma(\combelem)
      &=& \combgamma(\combelem) \cup \step \circ \combgamma(\combelem)\\
      &\subseteq& \combgamma(\combelem) \cup \combgamma \circ \combstep(\combelem)
      & (\because \; \text{condition~(\ref{equ:comb-sound2})})\\
      &\subseteq& \combgamma(\combelem \join \combstep(\combelem))
      & (\because \; \text{condition~(\ref{equ:comb-sound1})})\\
      &=& \combgamma \circ \combtransfer(\combelem)\\
    \end{array}
  \]
  Then, the abstract semantics $\combsem{\prog} = \underset{n \rightarrow
  \infty}{\lim}{(\combtransfer)^n(\icombelem)} $ is sound because it is defined
  with a sound abstract transfer function $\combtransfer$ using the combined
  one-step execution $\combstep$.
\end{proof}

Now, we have to show that two conditions (\ref{equ:comb-sound1})
and (\ref{equ:comb-sound2}) hold.
First, we prove the condition~(\ref{equ:comb-sound1}) as follows:
\begin{lemma}
  \[
    \forall \combelem_0, \combelem_1 \in \combdom. \; \combgamma(\combelem_0) \cup
    \combgamma(\combelem_1) \subseteq \combgamma(\combelem_0 \join \combelem_1)
  \]
\end{lemma}
\begin{proof}
  \[
    \begin{array}{cl}
      \multicolumn{2}{l}{
        \combgamma((\sabselem, \symbelem)) \cup \combgamma((\sabselem', \symbelem'))
      }\\
      =& \sgamma(\sabselem) \cup \symbgamma(\symbelem)
      \cup \sgamma(\sabselem') \cup \symbgamma(\symbelem')\\
      =& (\sgamma(\sabselem)\cup \sgamma(\sabselem'))
      \cup (\symbgamma(\symbelem) \cup \symbgamma(\symbelem'))\\
      \subseteq& \sgamma(\sabselem \join \sabselem')
      \cup (\symbgamma(\symbelem) \cup \symbgamma(\symbelem'))\\
      & \multicolumn{1}{r}{(\because \; \sabsdom \; \text{is sound})}\\
      =& \sgamma(\sabselem \join \sabselem')
      \cup \symbgamma(\symbelem \cup \symbelem')\\
      =& \combgamma((\sabselem \join \sabselem', \symbelem \cup \symbelem'))\\
      =& \combgamma((\sabselem, \symbelem) \join (\sabselem', \symbelem'))\\
    \end{array}
  \]
\end{proof}

To prove condition~(\ref{equ:comb-sound2}), we first prove the same property for
the sealed symbolic domain $\symbdom$ in Lemma~\ref{lemma:step-symb}.  Then, we
prove the properties of the $\reform$ function in Lemma~\ref{lemma:reform}.
Finally, we prove the condition~(\ref{equ:comb-sound2}) in
Lemma~\ref{lemma:comb-sound2}.

\begin{lemma}\label{lemma:step-symb}
  For a given set of pairs of abstract instantiation maps and sealed symbolic
  states $\symbelem \in \symbdom$, assume that the following condition is
  satisfied:
  \[
    \forall (\absimap, \symbst) \in \symbelem. \; \exists \symbst' \in
    \symbstset. \; \text{s.t.} \; \symbst \symbtrans \symbst'
  \]
  Then, the following property holds:
  \[
    \step \circ \symbgamma(\symbelem) \subseteq
    \symbgamma \circ \symbstep(\symbelem)\\
  \]
\end{lemma}
\begin{proof}
  \[
    \begin{array}{cl}
      \multicolumn{2}{l}{\step \circ \symbgamma(\symbelem)}\\
      =& \step(\bigcup \{ \instant{\symbst}{\absimap} \mid (\absimap, \symbst) \in
      \symbelem\})\\
      =& \{ \st' \mid (\absimap, \symbst) \in \symbelem \wedge \st \in
      \instant{\symbst}{\absimap} \wedge \st \trans \st'\})\\
      =& \{ \st' \mid (\absimap, \symbst) \in \symbelem \wedge \imap \in
      \imapgamma(\absimap) \wedge \instant{\symbst}{\imap} \trans \st'\})\\
      =& \{ \st' \mid (\absimap, \symbst) \in \symbelem \wedge \imap \in
      \imapgamma(\absimap) \wedge \instant{\symbst}{\imap} \trans \st'\\
       & \phantom{\{ \st' \mid (\absimap, \symbst) \in \symbelem \wedge \imap \in
      \imapgamma(\absimap)} \wedge \symbst \symbtrans \symbst' \})\\
      & \multicolumn{1}{r}{(\because \; \text{Assumption})}\\
      =& \{ \instant{\symbst'}{\imap} \mid (\absimap, \symbst)
      \in \symbelem \wedge \imap \in \imapgamma(\absimap) \wedge \symbst
      \symbtrans \symbst'\}\\
      & \multicolumn{1}{r}{(\because \; \text{Validity of} \; \symbtrans)}\\
      =& \bigcup \{ \instant{\symbst'}{\absimap} \mid (\absimap, \symbst)
      \in \symbelem \wedge \symbst \symbtrans \symbst' \}\\
      =& \symbgamma(\{ (\absimap, \symbst') \mid (\absimap, \symbst)
      \in \symbelem \wedge \symbst \symbtrans \symbst' \})\\
      =& \symbgamma \circ \symbstep(\symbelem)\\
    \end{array}
  \]
\end{proof}

\begin{lemma}\label{lemma:reform}
  For a given combined state $\combelem \in \combdom$, the $\reform$ function
  satisfies the following two properties:
  \begin{itemize}
    \item $\combgamma(\combelem) \subseteq \combgamma \circ \reform(\combelem)$
    \item $\forall (\absimap, \symbst) \in \symbelem. \; \exists \symbst' \in
      \symbstset.  \; \text{s.t.} \; \symbst \symbtrans \symbst'$
  \end{itemize}
  where $(\sabselem, \symbelem) = \reform(\combelem)$
\end{lemma}
\begin{proof}
  \[
    \fbox{$\combgamma(\combelem) \subseteq \combgamma \circ \reform(\combelem)$}
  \]
  \[
    \begin{array}{cl}
      \multicolumn{2}{l}{\combgamma((\sabselem, \symbelem))}\\
      =& \sgamma(\sabselem) \cup \symbgamma(\symbelem)\\

      =& \left( \underset{\view \in \viewset}{\bigcup} {\viewmap(\view) \cap
      \gamma \circ \sabselem(\view)} \right) \cup \left( \underset{(\absimap,
      \symbst) \in \symbelem}{\bigcup} \instant{\symbst}{\absimap} \right) \\

      =& \left( \underset{\view \in \viewset}{\bigcup} \aelemgamma((\view,
      \sabselem(\view))) \right) \cup \left( \underset{(\absimap, \symbst) \in
      \symbelem}{\bigcup} \aelemgamma((\absimap, \symbst)) \right) \\

      =& \dot\aelemgamma(\{ (\view, \sabselem(\view)) \mid \view \in \viewset \}
      \cup \symbelem)\\

      =& \dot\aelemgamma(\dot{\areform}(\{ (\view, \sabselem(\view)) \mid \view
      \in \viewset \} \cup \symbelem))\\

       & \multicolumn{1}{r}{(\text{Trivially,} \; \forall \aelem \in \aelemset.
       \; \aelemgamma(\aelem) = \aelemgamma \circ \areform(\aelem))}\\

      =& \dot\aelemgamma(E)\\
       & \multicolumn{1}{r}{(\text{See the definition of $E$ in
       Definition~\ref{def:reform}})}\\

      =& \left( \underset{(\view, \abselem) \in E}{\bigcup} \aelemgamma((\view,
      \abselem)) \right) \cup \left( \underset{(\absimap, \symbst) \in
      E}{\bigcup} \aelemgamma((\absimap, \symbst)) \right)\\

      =& \left( \underset{(\view, \abselem) \in E}{\bigcup} \viewmap(\view) \cap
      \gamma(\abselem) \right) \cup \left( \underset{(\absimap, \symbst) \in
      E}{\bigcup} \instant{\symbst}{\absimap} \right)\\

      =& \left( \underset{\view \in \viewset}{\bigcup} { \underset{(\view,
      \abselem) \in E}{\bigcup} \viewmap(\view) \cap \gamma(\abselem) } \right)
      \cup \left( \underset{(\absimap, \symbst) \in E}{\bigcup}
      \instant{\symbst}{\absimap} \right)\\

      =& \left( \underset{\view \in \viewset}{\bigcup} {\viewmap(\view) \cap
        \left(\underset{(\view, \abselem) \in
      E}{\bigcup}{\gamma(\abselem)}\right)} \right) \cup \left(
      \underset{(\absimap, \symbst) \in E}{\bigcup} \instant{\symbst}{\absimap}
      \right)\\

      \subseteq& \left( \underset{\view \in \viewset}{\bigcup} {\viewmap(\view)
        \cap \gamma\left( \underset{(\view, \abselem) \in E}{\bigjoin}\abselem
      \right)} \right) \cup \left( \underset{(\absimap, \symbst) \in E}{\bigcup}
      \instant{\symbst}{\absimap} \right)\\

      =& \sgamma\left( \lambda \view. \underset{(\view, \abselem) \in
      E}{\bigjoin}\abselem \right) \cup \symbgamma(E \cap (\absimapset \times
      \symbstset))\\

      =& \combgamma\left( \lambda \view. \underset{(\view, \abselem) \in
      E}{\bigjoin}\abselem, E \cap (\absimapset \times \symbstset) \right)

      = \combgamma \circ \reform((\sabselem, \symbelem))
    \end{array}
  \]
  \[\]
  \[
    \fbox{$\forall (\absimap, \symbst) \in \symbelem. \; \exists \symbst' \in
    \symbstset.  \; \text{s.t.} \; \symbst \symbtrans \symbst'$}
  \]

  For a given $(\absimap, \symbst) \in \symbelem$, there exists an analysis
  element $\aelem \in \aelemset$ such that $\areform(\aelem) = (\absimap,
  \symbst)$.  According to the definition of $\areform$ in
  Definition~\ref{def:areform}, there are two possible cases: $\aelem =
  (\absimap, \symbst) \wedge \exists \symbst' \in \symbstset. \; \text{s.t} \;
  \symbst \symbtrans \symbst'$ or $\aelem = (\view, \abselem) \wedge \aelem \in
  \Dom(\asconverter)$. We separately consider those two cases:
  \begin{itemize}
    \item $\aelem = (\absimap, \symbst) \wedge \exists \symbst' \in \symbstset.
      \; \text{s.t} \; \symbst \symbtrans \symbst'$\\
        By definition, $\exists \symbst' \in \symbstset.  \; \text{s.t} \;
        \symbst \symbtrans \symbst'$
    \item $\aelem = (\view, \abselem) \wedge \aelem \in \Dom(\asconverter)$\\
      By the condition~\ref{equ:asc-cond} in the Theorem~\ref{theorem:shortcut},\\
      $\exists k > 1. \symbst \symbtrans^k \excst$.  Thus, $\exists \symbst' \in
      \symbstset.  \; \text{s.t} \; \symbst \symbtrans \symbst'$
  \end{itemize}
\end{proof}


\begin{lemma}\label{lemma:comb-sound2}
  \[
    \forall \combelem \in \combdom. \; \step \circ \combgamma(\combelem) \subseteq
    \combgamma \circ \combstep(\combelem)\\
  \]
\end{lemma}
\begin{proof}
  \[
    \begin{array}{cl}
      \multicolumn{2}{l}{
        \step \circ \combgamma(\combelem)
      }\\
      \subseteq& \step \circ \combgamma((\sabselem, \symbelem))\\
       & \multicolumn{1}{r}{(\because \; \text{First property in
       Lemma~\ref{lemma:reform}}}\\
       & \multicolumn{1}{r}{\text{where} \; (\sabselem, \symbelem)
       = \reform(\combelem).)}\\

      =& \step(\sgamma(\sabselem) \cup \symbgamma(\symbelem))\\
      =& \step(\sgamma(\sabselem)) \cup \step(\symbgamma(\symbelem))\\
      \subseteq& \sgamma \circ \sabsstep(\sabselem) \cup \step(\symbgamma(\symbelem))\\
      & \multicolumn{1}{r}{(\because \; \sabsdom \; \text{is sound.})}\\
      \subseteq& \sgamma \circ \sabsstep(\sabselem) \cup \symbgamma \circ
      \symbstep((\symbelem))\\
               & \multicolumn{1}{r}{(\because \; \text{Sceond property in
               Lemma~\ref{lemma:reform}} }\\
               & \multicolumn{1}{r}{\text{and Lemma~\ref{lemma:step-symb}})}\\
      =& \combgamma((\sabsstep(\sabselem), \symbstep(\symbelem)))\\
      =& \combgamma \circ \combstep(\combelem)\\
    \end{array}
  \]
\end{proof}

\subsection{Termination}

First, let's define some notations.

\begin{itemize}
\item
Let's define initial state of combined domain as follows:
\[
  \icombelem = (\isabselem, \emptyset)
\]
\item
Let's define $\combelem^i$, $\sabselem^i$, and $\symbelem^i$ for $i \geq 0$ as follows:
\[
  \combelem^i = (\sabselem^i, \symbelem^i) = \combtransfer^i(\icombelem)
\]
which means resulting state after applying transfer function $\combtransfer \; i$ times.
\item
Let's define the lifted symbolic transition relation
$\liftsymbtrans \subseteq
(\absimapset \times \symbstset) \times (\absimapset \times \symbstset)$
as follows:
\[
  (\absimap, \symbst) \liftsymbtrans (\absimap, \symbst') \Leftrightarrow
  \symbst \symbtrans \symbst'
\]
\end{itemize}

\begin{theorem}[Termination]\label{theorem:termination}
  \[
    \exists n \in \numset. \forall m \geq n. \;
    \combelem^m = \combelem^n
  \]
\end{theorem}

We prove this theorem after proving a series of lemmas.
We first begin by showing that sensitive abstract interpretation terminates in
finite time.

\begin{lemma}[Termination of sensitive abstract interpretation]\label{lemma:sabs-term}
\label{theorem:sabs-termination}
  \[
    \exists n. \; \forall m \geq n. \;
    \sabselem^m = \sabselem^n
  \]
\end{lemma}

\begin{proof}
Note that for all $\sabselem, \sabselem' \in \sabsdom$ that satisfies
$\combtransfer((\sabselem, \_)) = (\sabselem', \_)$,
\[
  \begin{array}{rcl}
  \combtransfer((\sabselem, \_))
  &=& (\sabselem, \_) \join \combstep((\sabselem, \_))\\
  &=& (\sabselem, \_) \join (\_, \_) = (\sabselem \join \_, \_)\\
  &=& (\sabselem', \_)
  \end{array}
\]

which implies $\sabselem \order \sabselem'$.

Now, since $\combtransfer((\sabselem^i, \_)) = (\sabselem^{i+1}, \_),
\sabselem^i \order \sabselem^{i+1}$ holds for all $i$.
Then, $\sabselem^0 \order \sabselem^1 \order \sabselem^2 ...$ is an ascending chain.
By ascending chain condition, there exists n such that
for all $m \geq n, \sabselem^m = \sabselem^n$.
\end{proof}

Now, let's show that sealed static symbolic execution does terminate
given that sensitive abstract interpretation terminates.

We begin by defining the difference set $\diffset_i \in \symbdom$ for $i \geq 0$ as follows:
\[
  \diffset_i = \symbelem^{i+1} \setminus \symbelem^i
\]

For simplicity, we define $\diffset_i$ as $\emptyset$ for $i < 0$.
Then we prove its properties:
\begin{lemma}[Property of difference set]\label{lemma:diffset_prop}
  \[
    \begin{array}{c}
      \forall i \geq 0. \; \forall \symbaelem \in \diffset_i. \\
      \exists \view. \; \asconverter((\view,\sabselem^i(\view))) \liftsymbtrans \symbaelem 
      \lor \exists \symbaelem' \in \diffset_{i-1} . \; \symbaelem' \liftsymbtrans \symbaelem
    \end{array}
  \]
\end{lemma}
\begin{proof}
  Let $i \in \numset$ and $\symbaelem \in \diffset_i = \symbelem^{i+1} \setminus \symbelem^i$ given.
  By definition,
  \[
    \symbelem^{i+1} = \symbelem^i \cup \symbstep({\symbelem^i}')
  \]
  where
  \[
    (\_, {\symbelem^i}') = \reform(\sabselem^i, \symbelem^i)
  \]
  Note that $\symbaelem \in \symbstep({\symbelem^i}')$,
  and by definition of $\symbstep$, there exists some
  $\symbaelem' \in {\symbelem^i}'$ that satisfies $\symbaelem' \liftsymbtrans \symbaelem$.
  Now, by definition of $\reform$,
  \[
    {\symbelem^i}' =
    \dot{\areform}(\{ (\view, \sabselem^i(\view)) \mid \view \in \viewset \} \cup \symbelem^i)
    \cap (\absimapset \times \symbstset)
  \]
  This means there exists
  $\aelem \in \{ (\view, \sabselem^i(\view)) \mid \view \in \viewset \} \cup \symbelem^i$
  that satisfies $\areform(\aelem) = \symbaelem'$. We have two possible cases for $\aelem$.
  \begin{itemize}
 
  \item $\aelem \in \{ (\view, \sabselem^i(\view)) \mid \view \in \viewset \}$

  In this case, $\areform(\aelem) = \asconverter(\aelem) = \symbaelem'$
  and the left condition for conclusion is satisfied.
  
  \item $\aelem \in \symbelem^i$

  In this case, $\areform(\aelem) = \aelem = \symbaelem'$.
  Now, let's assume that $\aelem \in \symbelem^{i-1}$.
  In that case, $\aelem$ would be preserved after reform step, that is,
  $\aelem \in {\symbelem^{i-1}}'$. Then, by definition of $\symbstep$,
  $\symbaelem \in \symbstep({\symbelem^{i-1}}') \subseteq \symbelem^i$
  whcih contradicts to the fact that $\symbaelem \in \diffset_i$.
  Therefore, $\aelem \notin \symbelem^{i-1}$, that is,
  $\aelem \in \symbelem^i \setminus \symbelem^{i-1} = \diffset_i$,
  and the right condition for conclusion is satisfied.
  \end{itemize}
\end{proof}

\begin{corollary}\label{corollary:only-from-diffset}
  \[
    \begin{array}{c}
      \forall i > 0. \; \sabselem^{i-1} = \sabselem^i \Rightarrow
      \forall \symbaelem \in \diffset_i. \\
      \exists \symbaelem' \in \diffset_{i-1} . \; \symbaelem' \liftsymbtrans \symbaelem
    \end{array}
  \]
\end{corollary}
\begin{proof}
  The proof goes same as the previous lemma, until the point where we divide
  the case for $\aelem$. Let's assume that the first case holds, that is,
  \[
    \aelem \in \{ (\view, \sabselem^i(\view)) \mid \view \in \viewset \}
  \]
  Since $\sabselem^{i-1} = \sabselem^i$,
  \[
    \aelem \in \{ (\view, \sabselem^{i-1}(\view)) \mid \view \in \viewset \}
  \]
  In that case, $\aelem$ would be transformed after reform step, that is,
  $\asconverter(\aelem) = \symbaelem' \in {\symbelem^{i-1}}'$.
  Then, by definition of $\symbstep$,
  $\symbaelem \in \symbstep({\symbelem^{i-1}}') \subseteq \symbelem^i$
  whcih contradicts to the fact that $\symbaelem \in \diffset_i$.
  Therefore, only second case holds and the right conclusion in previus lemma is satisfied.
\end{proof}

Now, we can define the TTL(time to live) function
$\ttl_i: \diffset_i \rightarrow \numset$ for $i \geq 0$ as follows:
\begin{definition}[TTL Function]
  \[
    \begin{array}{c} 
      \ttl_i(\symbaelem) = \left \{
      \begin{array}{l}
        N - 1 \;\; ( \text{if} \; D = \emptyset)\\
        \text{min}(\dot\ttl_{i-1}(D)) - 1
        \;\; ( \text{otherwise})
      \end{array}
      \right. \\
      \\
      \text{where} \; D = 
      \{\symbaelem' \in \diffset_{i-1} \mid \symbaelem' \liftsymbtrans \symbaelem\}
    \end{array}
  \]
\end{definition}

We prove following properties of TTL function.
\begin{lemma}
  \[
    \begin{array}{c}
      \forall i \geq 0. \; \forall \symbaelem \in \diffset_i.
      \ttl_i(\symbaelem) = k \Rightarrow \\
      k < N \wedge
      \exists (\view, \abselem). \; (\asconverter((\view,\abselem))
      \liftsymbtrans^{(N - k)} \symbaelem) \\
    \end{array}
  \]
\end{lemma}
\begin{proof}
  We prove by induction on $i$.
  Let $\symbaelem \in \diffset_i$.
  \begin{itemize}
  \item If $i = 0$, $\ttl_0(\symbaelem) = N - 1 < N$
  and since only left conclusion of lemma~\ref{lemma:diffset_prop} can hold,
  there eixsts view $\view$ s.t.
  $\asconverter(\view, \sabselem^0(\view)) \liftsymbtrans^1 \symbaelem$.
  \item If $i > 0$, we have two cases for $D = 
    \{\symbaelem' \in \diffset_{i-1} \mid \symbaelem' \liftsymbtrans \symbaelem\}$.
  If $D = \emptyset$, the argument is similar as $i = 0$ case.
  Otherwise, let $\symbaelem' = \underset{\x \in D}{argmin}{\ttl_{i-1}(x)}$.
  
  By induction hypothesis, we have
  \[
    k' = \ttl_{i-1}(\symbaelem') < N
  \]
  and there eixsts $(\view, \abselem)$ such that
  \[
    \symbaelem'' = \asconverter((\view,\abselem)) \liftsymbtrans^{(N - k')} \symbaelem'.
  \]
  By definition of $\ttl_i$,
  $\ttl_i(\symbaelem) = \ttl_i(\symbaelem') - 1$, and $k = k' - 1$.
  Then,
  \[
    k = k' - 1 < N - 1 < N
  \]
  and
  $\symbaelem'' \liftsymbtrans^{(N - k - 1)} \symbaelem'$ with
  $\symbaelem' \liftsymbtrans \symbaelem$ implies that
  \[
    \symbaelem'' \liftsymbtrans^{(N - k)} \symbaelem.
  \]
  \end{itemize}
\end{proof}
\begin{corollary}\label{corollary:ttl-range}
  \[
    \forall i \geq 0. \; \forall \symbaelem \in \diffset_i. \;
    0 < \ttl_i(\symbaelem) < N
  \]
\end{corollary}
\begin{proof}
We already proved $k = \ttl_i(\symbaelem) < N$.
Now, let's assume that $k \leq 0$.
By previous lemma, there exists $(\view, \abselem)$ such that
\[
  (\asconverter((\view,\abselem)) \liftsymbtrans^{(N - k)} \symbaelem)
\]
Since $N - k \geq N$, this implies that there exists $\symbaelem'$ such that
\[
  (\asconverter((\view,\abselem)) \liftsymbtrans^N \symbaelem')
\]
However, this contradicts to the condition~(\ref{equ:asc-cond}) of $\asconverter$ that says
if $(\view,\abselem)$ is in domain of $\asconverter$,
the number of possible $\symbtrans$ from state of $\asconverter((\view,\abselem))$
is at most $N - 1$.
Therefore, $k > 0$.
\end{proof}

\begin{lemma}\label{lemma:ttl-decr}
  \[
    \begin{array}{c}
      \forall i > 0. \; \sabselem^{i-1} = \sabselem^i \Rightarrow \\
      sup(\dot \ttl_i(\diffset_i)) \leq sup(\dot \ttl_{i-1}(\diffset_{i-1})) - 1
    \end{array}
  \]
\end{lemma}
\begin{proof}
  Let $\symbaelem \in \diffset_i$.
  By Corollary~\ref{corollary:only-from-diffset}, the set
  \[
    D = \{\symbaelem' \in \diffset_{i-1} \mid \symbaelem' \liftsymbtrans \symbaelem\}
  \]
  is non-empty, and for some $\symbaelem' \in \diffset_{i-1}$,
  \[
    \ttl_i(\symbaelem) = \ttl_{i-1}(\symbaelem') - 1 \leq sup(\dot \ttl_{i-1}(\diffset_{i-1})) - 1
  \]
  Since it holds for every $\symbaelem \in \diffset_i$,
  \[
    sup(\dot \ttl_i(\diffset_i)) \leq sup(\dot \ttl_{i-1}(\diffset_{i-1})) - 1
  \]
\end{proof}

Now, we can complete the proof of the Theorem~\ref{theorem:termination}.

\begin{proof}
By Lemma~\ref{lemma:sabs-term}, there exists $n \in \numset$ s.t.
for all $m \geq n$,
\[
  \sabselem^m = \sabselem^n
\]
By Corollary~\ref{corollary:ttl-range},
\[
  sup(\dot \ttl_n(\diffset_n)) < N.
\]
Now, by Lemma~\ref{lemma:ttl-decr}, for all $i>0$,
\[
  sup(\dot \ttl_{n+i}(\diffset_{n+i})) \leq sup(\dot \ttl_{n+i-1}(\diffset_{n+i-1})) - 1
\]
which implies that
\[
  sup(\dot \ttl_{n+i}(\diffset_{n+i})) \leq sup(\dot \ttl_n(\diffset_n)) - i < N - i
\]
Therefore, for $j \geq N$,
\[
  sup(\dot \ttl_{n+j}(\diffset_{n+j})) < N - j \leq 0
\]
Notice that again by Corollary~\ref{corollary:ttl-range},
\[
  inf(\dot \ttl_{n+j}(\diffset_{n+j})) > 0
\]
meaning that
\[
  inf(\dot \ttl_{n+j}(\diffset_{n+j})) > sup(\dot \ttl_{n+j}(\diffset_{n+j}))
\]
which implies $\diffset_{n+j} = \emptyset$ and
$\symbelem^{n+j+1} = \symbelem^{n+j}$.

Therefore, for all $m \geq n + N$,
\[
  \sabselem^m = \sabselem^n \wedge \symbelem^m = \symbelem^n
\]
and
\[
  \combelem^m = \combelem^n
\]

\end{proof}

